Using Intermittent Synchronization to Compensate for Rhythmic Body Motion During Autonomous Surgical Cutting and Debridement

Anatomical structures are rarely static during a surgical procedure due to breathing, heartbeats, and peristaltic movements. Inspired by observing an expert surgeon, we propose an intermittent synchronization with the extrema of the rhythmic motion (i.e., the lowest velocity windows). We performed 2 experiments: (1) pattern cutting, and (2) debridement. In (1), we found that the intermittent synchronization approach, while 1.8x slower than tracking motion, was significantly more robust to noise and control latency, and it reduced the max cutting error by 2.6x In (2), a baseline approach with no synchronization achieves 62% success rate for each removal, while intermittent synchronization achieves 80%.

==> 3-stewart.tex <==

\iffalse
\section{Stewart Platform: Technical Description}
This section describes the miniature Stewart platform. Our design and control of the platform reference \cite{stewartMath} for the kinematics and \cite{stewartInstructable} for manufacturing.

\begin{figure}[b]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/StewartV2_Render1.png}
    \caption{Rendered CAD model of the second iteration of the Stewart platform. The bottom structure (purple) and the top platform (cyan) were constructed from 1/4 inch laser cut acrylic sheets, and the servo horns (yellow) and buttress support (orange) were made from 1/4 inch Delrin sheets. The Dynamixel XL-320 servos (grey),  and support rods (red) were purchased parts.}
    \label{render_platform}
    \renewcommand{\bottomfraction}{0.15}
\end{figure}


\subsection{Motivation and Design Considerations}

The physical and dynamic design of the platform was driven by two specific needs; to (1) to have a range of motion capable of replicating a variety of organ motions and (2) to fit and interact in the preexisting testing setup of the AUTOLAB da Vinci Research Kit (DVRK). Since internal organs have small ranges of motion \cite{Gagne2014}, we were able to keep the device compact by defining a small desired range of motion.  Additionally, the main constraint regarding physical dimensions was the 21.6 cm between the table of the workspace and the endoscopic stereo camera, driving the device to require a thin vertical profile. Thus, to address (1) and (2), the maximum vertical motion range of the platform was aimed to be under $\pm$ 12.7 cm from a set home position and the maximum rotational range of the platform was chosen to be at most $\pm$ $15^{o}$. Fitting under these design constraints, the maximum and minimum vertical height of the device was 11.4 and 9.5 cm respectively.  To further address (2), the platform had an equally wide base and platform to accommodate our larger surgical simulation tools. Figure \ref{platformDim} shows the dimensions listed in Table \ref{dim_platform} for the platform designed with these particular requirements in mind.

% Top Plate design: hollow, modular attachments, wide workspace
Unique to our design was the platform's modular testing surface. Different removable work surfaces can be attached to the main platform by being screwed into a series of preset holes (Figure \ref{attach_platform}). An assortment of work surfaces can be created and customized for different surgical tasks and swapped in and out quickly, rather than being constrained to one work surface. It should be pointed out that the device's main top plate was designed with a hollow center. This was done intentionally to prevent any damage to the DVRK's end effectors and to the platform itself, when performing tasks during testing. Moreover, the platform is made up entirely of off-the-shelf parts and easily fabricated components from cheap materials. Most of these parts can also be swapped easily if damaged. Especially in a research and training setting where failures are more common, a cost-effective tool like this platform becomes even more valuable.

% Second version purpose and details of changes
A second version of the Stewart platform displayed in Figure \ref{render_platform} was made to address some of the limitations of the first version such as the physical restrictions on the range of motion, jittery and inaccurate servo motion, and complicated pulse width modulation control. The HI-TEC HS422 servos were replaced with Dynamixel XL-320 servos, and the Teensy micro-controller was swapped for the OpenCM 9.04C controller. The new servos were controlled with digital packets so they offered faster and repeatable motion at a higher resolution. The new version also swapped the servo supports for rivets, and used a redesigned servo horn to prevent the rods from coming in contact with any components and limiting the range of motion. The code on the micro-controller and scripts used for serial communication were modified to account for the characteristics of the new servos.

%The main structure of the AUTOLAB Stewart platform (purple, cyan, and orange in Figure \ref{render_platform}) was manufactured from 1/4 inch acrylic using a Universal Laser VLS 6.6 laser cutter. 

%Table \ref{material_platform} provides the full material list of our main platform, 
%\begin{table}[]
%\centering
%\caption{Material List for Platform}
%\label{material_platform}
%\begin{tabular}{lcl}
%\hline
%\textbf{Part Name}                   & \multicolumn{1}{l}{\textbf{Quantity}} & \textbf{Note}                     \\ %\hline
%    1/4 inch Acrylic Sheet           & ---                                   & laser cut to shape       \\
%    HS-422 Deluxe Standard Servo     & 6                                     &                          \\
%    Aluminum servo horns             & 6                                     &                          \\
%    Teensy 3.2 Microcontroller       & 1                                     &                          \\
%    2.5 inch m3 pushrods             & 6                                     & cut to length         \\
%    1/4 inch Delrin pieces           & 12                                    & laser cut to shape,   \\
%                                     &                                       & tapped for pushrods   \\
%    Nylon Ball-joints                & 12                                    &                          \\
%\end{tabular}
%\end{table}


\begin{table}[]
\centering
\caption{Important Platform Dimensions used in the miniature Stewart Platform, referenced from Figure \ref{platformDim} }
\label{dim_platform}
\begin{tabular}{cll}
\textbf{Variable}                 & \textbf{Value}                       & \multicolumn{1}{c}{\textbf{Description}}        \\ \hline \hline
    L1                            & 2.0 cm                             & servo arm length      \\
    L2                            & 6.0 cm                             & platform linkage length       \\
    $Z_{home}$                    & 5.1 cm                              & platform height above servo axis (linkages at $90^{o}$)  \\
    $L_{OB}$                      & 8.1 cm                            & length $O$ to platform attachment points $P_{i}$          \\
    $L_{OP}$                      & 8.1 cm                            & length $O$ to servo attachment points $B_{i}$ \\
    $\theta_{b}$                  & $31^\circ$                          & angle between servo axis attachment points \\
    $\theta_{p}$                  & $23.5^\circ$                          & angle between platform attachment points    \\
\end{tabular}
\end{table}



\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/stewart_attach_small3.png}
    \caption{(1) Three attachment points on the Stewart platform (2) Attachment with clips for gauze (3) Makeshift attachment for gauze-wrapped silicone phantoms used in this paper (Figure \ref{exp-setup})}
    \label{attach_platform}
    \renewcommand{\bottomfraction}{0.5}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=0.7\columnwidth]{figures/dim_platform.png}
    \caption{Reference for dimensions of the platform. The top image is a top view and the bottom image is a side view. The platform is depicted in red and the base is depicted in blue.}
    \label{platformDim}
    \renewcommand{\bottomfraction}{0.5}
\end{figure}




%\subsection{Inverse Kinematics}



\subsection{Software Interface}

The platform has two preset motion modes available for each degree of freedom.  The first available mode is sinusoidal motion, governed by:
% Sine Wave
\[ y(t) = A\sin(2 \pi \omega t)\]
%
The second mode simulates breathing-inspired motion, motivated by \cite{stewartBreathe}. Breathing motion is defined as:
%
% Sine Breathe
% for xyz
\[ y(t) = \Big( exp(\sin(\omega t)) - \frac{1}{e} \Big) \frac{2A}{e-\frac{1}{e}}\]
%
%and rotational breathing motion is described by:
%
% for rpy, subtract amplitude to osicallate about zero
%\[ y(t) = \Big( exp(\sin(\omega t)) - \frac{1}{e} \Big) \frac{2A}{e-\frac{1}{e}} - A\]
%
where $A$ is amplitude and $\omega$ is frequency. 
%In the breathing motion equation, a whole "breath" oscillates about the defined amplitude. 
For rotational motion, the amplitude $A$ is subtracted from the wave so a "breath" oscillates about each axis, rather than the defined amplitude value.

%In addition to these modes, custom positions and rotations can be commanded to the platform.

% From ARDUINO
%sinWave
%  arr[2] = ampZ*sin(2*pi*freqZ*T);
%  arr[3] = radians(ampX_rot*sin(2*pi*freqX_rot*T));

%sinBreathe
%  arr[2] = (exp(sin(freqZ*T)) - 1/exp(1))*((2*ampZ)/(exp(1)-(1/exp(1))));
%  arr[3] = radians(((exp(sin(freqX_rot*T)) - 1/exp(1))*((2*ampX_rot)/(exp(1)-(1/exp(1)))))-ampX_rot);

\fi

==> dump-arch.tex <==
\section{Problem Statement and Overview}
In this section, we overview the system architecture, assumptions, and inputs and outputs of each component.

\subsection{Problem Statement}
We consider a generalization pattern cutting tasks from Fundamentals of Laparoscopic Surgery (FLS), which is a standard training regimen for medical students in laparoscopic surgery~\cite{Ritter2007}. A typical pattern cutting task features a 50~mm diameter, 2~mm thick circular pattern marked on a 4$\times$4~inch square of standard surgical gauze suspended by clips and that it lies in the horizontal plane. 
We consider a generalization where the gauze is marked with an arbitrary curve that does not self-intersect.

We assume that one arm of the robot is designated as the cutting arm and one is the tensioning arm.
The tensioning arm applies tension to the gauze from a fixed grasping point.
The task is complete once the pattern has been cut from the surrounding gauze.

\subsection{Algorithm Overview}

\begin{enumerate}
    \item \textbf{Inputs: } Parametric planar curve $c(t)$
    
    \item \textbf{Outputs: } Cutting Trajectory $k(t)$, Grasping Points $(x,y)$, Tensioning Policy $\pi$
\end{enumerate}




\vspace{0.25em}

\noindent\textbf{1. Generate Cutting Paths: } Given the registered pattern, represented parametrically by a finite sequence of points, and the kinematic constraints of the da Vinci arm, we automatically generate a fully executable path for cutting. Depending on the pattern, this reachable trajectory may be composed of separate segments such that few temporally adjacent points in the trajectory are non-contiguous. Our heuristic divides the original pattern into segments by determining notch points, or the locations on the pattern where the scissors must begin a new cut, and end points. 

Let us initially assume (will relax subsequently) that the tensioning point is given.
Given this cutting trajectory a first approach would be to always tension orthogonally to the cut.
However, as more of the gauze is cut, the fabric will transfer the tension along multiple distinct paths--making it hard to predict the effect of the tension at the point of cut.
\todo{We highlight this point in our simulated experiments, where we find that on some curves the orthogonal tensioning performs worse than no tensioning at all.}
The tensioning policy needs to be aware of the gauze's deformation and the current progress of the cutting arm.
Since this deformation is difficult to model analytically, Reinforcement Learning (RL) is a viable option.
However, the number of trials run in exploration can be very high, which may not be practical in Patter Cutting because of the cost of resetting failed trials.  
This paper explores the feasibility of a fabric simulator to train an adaptive tensioning policy.

For a tensioning policy and cut trajectory pair, the simulator returns a quality score using the symmetric difference.
Let $X$ be the set of points inside a closed intended trajectory and let $Y$ be the set of points inside a closed simulated trajectory. The symmetric difference is then simply the exclusive-or $A \oplus B$ of the two sets. Open curves are treated as closed curves by forming boundaries with the edges of the cloth.

We can use this quality score to select a grasping point.
We try many random grasping points calculate the tensioning policy and cut trajectory pair and evaluate the quality score with the simulator and select the grasp point that leads to the highest score overall.
\todo{We evaluated learned tensioning policy in physical experiments on the  da Vinci Research Kit (DVRK). 
The simulator is registered to the gauze using colored fiducial points tracked with a computer vision system.}





==> simulator.tex <==

\section{Simulator}
\label{simulator}
A planar fabric can be modeled as a rectangular mesh of vertices. 
These vertices move independently in the x,y,z coordinates governed by forced differential equations.
Suppose, each vertex $(i,j)$ of the fabric has coordinates $p_{ij}^{(x)},p_{ij}^{(y)},p_{ij}^{(z)}  \in \mathbf{R}$, and in isolation, each follows the following equations of motion:
\[
\ddot{p}_{ij} = \alpha p_{ij}  + \delta \dot{p}_{ij} + f(t)
\]
The interaction between the vertices is governed by the tensile modulus $\tau$ acting as an ideal spring:
\[
\ddot{p} = \alpha p  + \delta \dot{p} - \sum_{p' \in \text{neighbors}} \tau (p' - p)  + f(t)
\]
To model cutting, we remove a point from the set of vertices.
\[
\ddot{p} = \alpha p  + \delta \dot{p} - \sum_{p' \in \text{neighbors} \land \neg \text{cut}} \tau (p' - p)  + f(t)
\]
To model standard surgical gauze, we use the following parameters $\delta = 0.008$, $\alpha=0.99$, $\tau=1.0$ and $f(t)$ is gravity.
We fit these parameters through trial and error, observing how cutting trajectories deformed in real gauze vs. the simulator.

We use 625 vertices (25 x 25) in our experiments to approximate the physical gauze. Each time step requires an update of each vertex's location due to external forces such as gravity and internal forces represented by the constraints between adjacent vertices. Running this simulator with many iterations in each run is relatively expensive, so we took several steps to maintain a runtime that would allow both suitable approximation of the cloth and fast computation for update steps. 
We compiled our Python code using the Python package Cython to write C extensions. This sped up each run of the simulation by a factor of six, which allowed us to run tens of thousands of simulations in a reasonable amount of time.\todo{sk. explain}. 

%\todo{change to the symmetric difference: To quantify the effectiveness of the trajectory planning and tensioning policy, we implemented a simple scoring scheme. The subset of vertices approximating the given pattern is tagged as \textit{shape points}. An uncut cloth is given an initial score which reflects the number of shape points in the uncut pattern. Once a simulation is complete, meaning the planned trajectory is executed in full, our code generates a final score directly proportional to the number of shape points that have not been separated or, rather, cut from normal unmarked points}. We then attempt to minimize the score, finding the best trajectory and tensioning policy with which it corresponds.

\subsection*{Step 1. Plan Trajectory}


\subsection*{Step 2. Learn Tensioning Policy}
Using the optimal order of segments, we can arrive at a trajectory for the cutting arm $\chi(n)$ for $n \in \{1,...,N\}$.
Now, our goal is to plan a policy for the tensioning arm, such that this trajectory follows the marked curve as closely as possible.
We model the tensioning problem as a Markov Decision process $\mathcal{M}$:
\[
\mathcal{M} = \langle S,A,T(\cdot,\cdot), R(\cdot,\cdot),N \rangle.
\]
The state-space is defined as a four-tuple consisting of the time index of the trajectory and the displacement vector from the original gripper tensioning location, and the actions are 1mm movements in each of the cardinal directions.
The reward function is the indicator function:
\[
R(s,a) = \mathbf{I}(\chi(n))
\]
which measures whether the next cut applied in the trajectory lands on a marked point on the curve.
The objective is to find a policy $\pi: S \mapsto A$ that optimizes this reward function.

\subsection*{Step 3. Execute}
The da Vinci Research Kit (DVRK) is a development
platform provided by Intuitive Surgical to advance research in teleoperated robotic surgical systems. We use two tools: the Large Needle Driver and the Curved Scissors.
The Large Needle Driver is a grasper with 6 mm fingers (tensioning arm).
The Curved Scissors are a cutting instrument 10 mm in length (cutting arm).
Given the plan $\chi(n)$  and the tensioning policy $\pi$, we execute this on the robot.
Of course, the simulator is an approximation of the true model and the actual execution of the policy on the real gauze will differ from the simulation.
To address this problem, we apply visual position control in addition to the tensioning policy.
